SDSS-IV MaNGA: Star formation cessation in low-redshift galaxies I. Dependence on stellar mass and structural properties

We investigate radial gradients in the recent star formation history (SFH) using 1917 galaxies with $0.01<z<0.14$ and integral-field spectroscopy from the ongoing MaNGA survey. For each galaxy, we obtain two-dimensional maps and radial profiles for three spectroscopically-measured parameters that are sensitive to the recent SFH: D$_n$(4000) (the 4000\AA\ break), EW(H$\delta_A$) (equivalent width of the H$\delta$ absorption line), and EW(H$\alpha$) (equivalent width of the H$\alpha$ emission line). We find the majority of the spaxels in these galaxies are consistent with models with continuously declining star formation rate, indicating that starbursts occur rarely in local galaxies. We classify the galaxies into three classes: fully star-forming (SF), partly quenched (PQ) and totally quenched (TQ), according to the fraction of quenched area within 1.5 times the effective radius, $f_Q(1.5R_e)$. We find that galaxies less massive than $10^{10}$M$_{\odot}$ present at most weak radial gradients in all the diagnostic parameters. In contrast, galaxies with stellar mass above $10^{10}$M$_{\odot}$ present significant gradients in all the three diagnostic parameters if classified as SF or PQ, but show weak gradients in D$_n$(4000) and EW(H$\delta_A$) and no gradients in EW(H$\alpha$) if in the TQ class. This implies the existence of a critical stellar mass, at $\sim10^{10}$M$_{\odot}$, above which the star formation in a galaxy gets shutdown from the inside out. Galaxies tend to evolve synchronously from inner to outer regions before their mass reaches the critical value. We have further divided the sample at fixed mass by both bulge-to-total luminosity ratio and morphological type, finding that our conclusions hold regardless of these factors: it appears that the presence of a central dense object is not a driving parameter, but rather a byproduct of the star formation cessation process.

==> makefile <==
SOURCE = ms

.SUFFIXES:	.aux .dvi .ps .tex

# edit and process the .tex file
default:	twice ps 
#gv

main:		$(SOURCE).aux
			latex $(SOURCE)
dvi:		$(SOURCE).dvi
ps:			$(SOURCE).ps
once:
			latex $(SOURCE)
twice:		once once
			latex $(SOURCE)
bib:		
			bibtex $(SOURCE)

x:			$(SOURCE).dvi
			xdvi -geometry +0+0 -s 8 -bg white -fg black \
			-expert -hush $(SOURCE).dvi &
gv:			$(SOURCE).ps
			gv $(SOURCE).ps &


.dvi.ps:
			dvips -f $< > $(SOURCE).ps
.tex.aux:
			latex $(SOURCE)	# create .aux file from $<
.tex.dvi:
			latex $<	# create .dvi file from $<

clean:	
			rm -f *~ *.log *.dvi *.aux *.blg  *.lof *.lot *.toc *.bbl *~ 
cleanest:	
			rm -f *~ *.log *.dvi *.ps *.aux *.toc *.bbl *.blg *.lot


